Towards enhanced performance in fusion plasmas via turbulence suppression by MeV ions

Megaelectron volt (MeV) alpha particles will be the main source of plasma heating in magnetic confinement fusion reactors. Yet, instead of heating fuel ions, most of the energy of alpha particles is transferred to electrons. Furthermore, alpha particles can also excite Alfvenic instabilities, previously considered as detrimental. Contrary to expectations, we demonstrate efficient ion heating in the presence of MeV ions and strong fast-ion driven Alfvenic instabilities in recent experiments on the Joint European Torus (JET). Detailed transport analysis of these experiments with state-of-the-art modeling tools explains the observations. Here we show a novel type of turbulence suppression and improved energy insulation in plasmas with MeV ions and fully developed Alfvenic activities through a complex multi-scale mechanism that generates large-scale zonal flows. This mechanism holds promise for a more economical operation of fusion reactors with dominant alpha particle heating and, ultimately, cheaper fusion electricity

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
